The Standard Aspect of Dialectical Logic

Dialectical logic is the logic of dialectical processes. The goal of dialectical logic is to introduce dynamic notions into logical computational systems. The fundamental notions of proposition and truth-value in standard logic are subsumed by the notions of process and flow in dialectical logic. Dialectical logic has a standard aspect, which can be defined in terms of the "local cartesian closure" of subtypes. The standard aspect of dialectical logic provides a natural program semantics which incorporates Hoare's precondition/postcondition semantics and extends the standard Kripke semantics of dynamic logic. The goal of the standard aspect of dialectical logic is to unify the logic of small-scale and large-scale programming.

==> nets.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Examples}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Hyperdoctrines.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We discuss here the very important example of ``dialectical functional spans (hyperdoctrines)''.

The ``action'' of a term $\term{y}{r}{x}$ is concentrated in and localized to a ``locus of activity'',
a source subtype called the domain-of-definition of $r$
(and a target subtype called the range of $r$).
This domain is a kind of ``effect'' or ``read-out'' of a term $r$,
and defines predicate transformation so that $r$ becomes a predicate transformer.

We assume that we are in a spannable join bisemilattice {\bf P} which has type sums.
For any type $x$ let $\widehat{\Omega^\dashv}(x)$ denote $x$-comonoids
in the join bisemilattice $\widehat{{\bf P}^\dashv}$.
These are diagonal functional spans of the form
$\phi = (x \stackrel{f \dashv f^{\rm op}}{\leftharpoondown} y \stackrel{f \dashv f^{\rm op}}{\rightharpoondown} x)$,
and can be identified with functional terms $\term{y}{f \dashv f^{\rm op}}{x}$ into $x$.
By definition of $\widehat{\Omega^\dashv}(x)$,
the underlying {\bf P}-term operator
$\widehat{{\rm P}^\dashv}[x,x] \stackrel{\uterm{x}{x}}{\longrightarrow} {\bf P}[x,x]$
restricts to comonoids:
for any diagonal functional span $\phi$ as above,
the underlying {\bf P}-term is
$\flat_x(\phi) =  \uterm{x}{x}(\phi) = f^{\rm op} \tprod f$,
the comonoid associated with the functional term
$\term{y}{f \dashv f^{\rm op}}{x}$.  
So $\flat_x$ is the {\em associated comonoid\/} operator.
Analogous to the term/span reflective pair $\utermspano{x}{x} = (\uterm{x}{x} \dashv \spano{x}{x})$,
we assume the existence of a right adjoint left inverse
$\widehat{\Omega^\dashv}(x) \stackrel{\sharp_x}{\longleftarrow} \comonoid{}{(x)}{}$
to the associated comonoid operator $\flat_x$.
This means existence of a reflective pair 
$\widehat{\Omega^\dashv}(x) \stackrel{\natural_x}{\longrightarrow} \comonoid{}{(x)}{}$
of monotonic functions $\natural_x \define (\flat_x \dashv \sharp_x)$.
We assume that the reflective pair $\natural_x$ and the term/span reflective pair $\utermspano{x}{x}$
commute with the inclusion/interior coreflective pairs,
forming a commuting square
\begin{center}
   $\begin{array}{ccc}
       \widehat{\Omega^\dashv}(x)
       & 
       \makebox{\rule{.1in}{0in}}
       \makebox[0in]{\raisebox{.12in}[0in][0in]{\scriptsize$\natural_x$}} \makebox[0in]{$\longrightarrow$}
       \makebox{\rule{.1in}{0in}}
       &
       \comonoid{}{(x)}{}
       \\
       \makebox[0in][r]{\scriptsize${\rm Inc} \dashv \interior{(\,)}$} \downarrow
       &
       & \downarrow \makebox[0in][l]{\scriptsize${\rm Inc} \dashv \interior{(\,)}$}
       \\
       \widehat{{\rm P}^\dashv}[x,x]
       &
       \makebox[0in]{\raisebox{-.12in}[0in][0in]{\scriptsize$\utermspano{x}{x}$}} \makebox[0in]{$\longrightarrow$}
       &
       {\bf P}[x,x]
    \end{array}$
\end{center}
for any type $x$.
This implies that $\sharp_x$ must be defined by
$\sharp_x = {\rm Inc} \cdot \spano{x}{x} \cdot \interior{(\,)}$,
and must satisfy the equality
$\sharp_x \cdot \flat_x = {\rm Id}$;
so that for any $x$-subobject $\term{y}{f \dashv f^{\rm op}}{x}$ 
and any $x$-comonoid $u \memberof \comonoid{}{(x)}{}$,
we have the equivalence
$\flat_x(\term{y}{f \dashv f^{\rm op}}{x}) \preceq u$
iff
$(\term{y}{f \dashv f^{\rm op}}{x}) \preceq (\term{x}{e \dashv e^{\rm op}}{x})$
where $\sharp_x(u) = \term{z}{e \dashv e^{\rm op}}{x}$ and $e^{\rm op} \tprod e = u$
iff
there is a functional term
$\term{y}{h \dashv h^{\rm op}}{z}$
such that $f = h \tprod e$ and $e^{\rm op} \tprod h^{\rm op} = f^{\rm op}$.
So we can interpret $\sharp_x(u)$ to be the ``largest'' $x$-subobject
whose associated comonoid is $u$.
Interpreting in terms of graphs,
for any {\bf P}-comonoid $u \memberof \comonoid{}{(x)}{}$
with overlying span (${\bf P}^\dashv$-graph)
$\spano{x}{x}(u)
 = (x \stackrel{p_0 \dashv p_0^{\rm op}}{\leftharpoondown} y \stackrel{p_1 \dashv p_1^{\rm op}}{\rightharpoondown} x)$
we must have
$\sharp_x(u)
 = \term{z}{e \dashv e^{\rm op}}{x}
 = (x \stackrel{e \dashv e^{\rm op}}{\leftharpoondown} z \stackrel{e \dashv e^{\rm op}}{\rightharpoondown} x)$ 
the equalizer (self-loops) of this ${\bf P}^\dashv$-graph.
Moreover,
$e^{\rm op} \tprod e = p_0^{\rm op} \tprod p_1 = u$.
So $u$ specifies self-loops for ${\bf P}^\dashv$-graphs.

%$\spano{x}{x}$ maps {\bf P}-comonoids to diagonal functional spans ($\widehat{{\rm P}^\dashv}$-comonoids).
%which commute with inclusions of comonoids as endoterms
%(``cut down'' to comonoids),
%and $\sharp_x(u) = \spano{x}{x}(u)$

In particular,
$\spano{}{}$ preserves identities
$\spano{x}{x}(x) = 
 (x \stackrel{x \dashv x}{\leftharpoondown} x \stackrel{x \dashv x}{\rightharpoondown} x)$.

Our approach regards the notion of domain-of-definition as fundamental,
and defines totalness as a derived notion.
The {\em domain subtype\/} of any term $\term{y}{r}{x}$
is the source subtype $\domain{(r)} = \term{d_r}{i_r \dashv p_r}{y}$
which satisfies the axioms:
(1) ``minimality''
    $z \succeq \domain{(r)}$ iff $p \circ i \circ r = r$
    for any source subtype $\term{z}{i \dashv p}{y}$;
(2) ``composition''
    $\domain{(s \circ r)} = \domain{(s \circ p_r)}$
    for any composable term $\term{z}{s}{y}$; and
(3) ``monotonicity''
    $r \preceq r'$ implies $\domain{(r)} \preceq \domain{(r')}$
    for any parallel term $\term{y}{r'}{x}$.
Define the {\em totalization\/} of $r$ to be the $r$-subterm $\total{r} \define i_r \circ r$.
A term $\term{y}{r}{x}$ is {\em total\/}
when its domain is the largest source subtype,
the entire source type $\domain{(r)} = y$.
Some identities for the domain operator $\domain{}$ are:
types are their own domain
$\domain{(x)} = x$;
the totalization is total, since
$\domain{(\total{r})}
 = \domain{(i_r \circ r)}
 = \domain{(i_r \circ p_r)}
 = \domain{(d_r)}
 = d_r$;
functional terms $\term{y}{f \dashv f^{\rm op}}{x}$ are total,
since the counit inequality $y \preceq f \circ f^{\rm op}$ implies
$y = \domain{(y)}
 \preceq \domain{(f \circ f^{\rm op})}
       = \domain{(f \circ p_{f^{\rm op}})}
 \preceq \domain{(f \circ x)}
       = \domain{(f)}
 \preceq y$;
in particular,
subtypes are total
$\domain{(\term{y}{i \dashv p}{x})} = y$;
domain subtypes are their own domain, since
$\domain{(p_r)}
 = \domain{(p_r \circ d_r)}
 = \domain{(p_r \circ \total{r})}
 = \domain{(r)}
 = d_r$;
only zero has empty domain
$\domain{(r)} = \term{0}{\bot_{0,y} \dashv \bot_{y,0}}{y}$
iff $r = 0_{y,x}$ for any term $\term{y}{r}{x}$; and
given any two total terms $\term{z}{s}{y}$ and $\term{y}{r}{x}$,
the composite term $\term{z}{s \circ r}{x}$ is also total,
since 
$\domain{(s \circ r)}
 = \domain{(s \circ p_r)}
 = \domain{(s \circ y)}
 = \domain{(s)}
 = z$.

The {\em domain subobject\/} of any term $\term{y}{t}{x}$
is the source subobject
$d_t \stackrel{i_d \dashv p_d}{\rightharpoondown} y$
where the term $t$ has non-nil action. 
The domain subobject (if it exists) is the ``smallest'' source subobject
such that the term $t$ is recoverable from the associated subterm by the identity
$t = (p_d \tprod i_d) \tprod t$;
so that, 
$t \preceq v \tprod t$
iff $\flat_y(d_t \stackrel{i_d \dashv p_d}{\rightharpoondown} y) \preceq v$
iff $(d_t \stackrel{i_d \dashv p_d}{\rightharpoondown} y) \preceq \sharp_y(v)$
for any source comonoid $v \memberof \comonoid{}{(y)}{}$.
The associated $t$-subterm
$t^\dagger = i_d \tprod t$ 
is called the {\em totalization\/} of $t$.
The term $t$ and its totalization $t^\dagger$ are equivalent by the identities
$\left\{\begin{array}{r@{\;=\;}c@{\;=\;}l}
           t         & p_d \tprod t^\dagger & {\bf P}^{[i_d,x]}(t^\dagger) \\
           t^\dagger & i_d \tprod t         & {\bf P}_{[i_d,x]}(t)
        \end{array} \right\}$.
A term $t$ is {\em total\/} when its domain subobject is the total source type $d_t = y$;
and then $t^\dagger = t$.

Total terms are close above w.r.t. term entailment order.
Since functional terms (in particular, identity terms) are total,
and the composite of total terms are also total,
total terms form a biposet $\total{{\bf P}}$,
a subbiposet of ${\bf P}$,
${\bf P}^\dashv \subseteq \total{{\bf P}} \subseteq {\bf P}$,
which is the homset order closure of ${\bf P}^\dashv$.
So $\total{{\bf P}}$ is a subbiposet ${\bf P}$,
which preserves homset joins but usually does not have a bottom.
Total terms in Heyting categories have been suggested \cite{Hoare} (although not by that name)
as good models for programs
(brief discussion in the section on Heyting categories).

%In the classical case,
%the domain $d \stackrel{i_d \dashv p_d}{\rightharpoondown} y$ of a term $\term{y}{r}{x}$ has a ``complement'',
%a $y$-subtype $k \stackrel{i_k \dashv p_k}{\rightharpoondown} y$ called the {\em kernel\/} of $r$,
%whose associated $r$-subterm is empty $i_k \circ r = \bot_{k,x}$. 
%The source type $y$ is a type sum $y = d \oplus k$ of the domain and kernel subtypes,
%and satisfies the disjointness identities
%$\bot_{d,k} = i_d \circ p_k$ and $\bot_{k,d} = i_k \circ p_d$,
%or the comonoid disjointness equation
%$(p_d \circ i_d) \circ (p_k \circ i_k) = \bot_y$,
%or better the negation identity
%$\boolneg{(p_d \circ i_d)} = (p_k \circ i_k)$.
%The {\em domain/kernel decomposition\/} of term $r$
%consists of the domain and kernel subtypes $d$ and $k$,
%plus the totalization subterm $\total{r}$.

Given any {\bf C}-arrow $y \stackrel{h}{\rightarrow} x$,
composition defines a direct image monotonic function
${\bf Sub}(y) \stackrel{\exists^\ast_h}{\longrightarrow} {\bf Sub}(x)$
where $\exists^\ast_h(z \stackrel{g}{\rightarrow} y) = g \cdot_C h$,
and an inverse image monotonic function
${\bf Sub}(y) \stackrel{{\rm sub}^\ast_h}{\longleftarrow} {\bf Sub}(x)$
where ${\rm sub}^\ast_h(w \stackrel{f}{\rightarrow} x) = \hat{w} \stackrel{\hat{f}}{\rightarrow} y$
the pullback of $f$ along $h$.

It is easy to check that $\widehat{\bf C}$ 
has both domains and ranges,
with $\domain{(\rho)} = (y \stackrel{r_0}{\leftarrow} r \stackrel{r_0}{\rightarrow} y)$
and  $\range{(\rho)}  = (x \stackrel{r_1}{\leftarrow} r \stackrel{r_1}{\rightarrow} x)$
for any span $\rho = (y \stackrel{r_0}{\leftarrow} r \stackrel{r_1}{\rightarrow} x)$;
so it has direct Hoare flow $\directsquare{\rho}{}$ defined by
$\directsquare{\rho}{(\psi)}
 \define  \range{(\psi \tprod \rho)}
       =  \exists^\ast_{r_1}({\rm sub}^\ast_{r_0}(g))$
for any $y$-comonoid $\psi = (y \stackrel{g}{\leftarrow} z \stackrel{g}{\rightarrow} y)$.
With the obvious involution $\widehat{\bf C}$ is an involutive direct Hoare flow category;
so it has dual direct Hoare flow $\directdiamond{\rho}{}$ defined by
$\directdiamond{\rho}{(\psi)}
 = \directsquare{{\rho}^{\rm op}}{(\psi)}
 = \domain{(\rho \tprod \phi)}
 = \exists^\ast_{r_0}({\rm sub}^\ast_{r_1}(f))$
for any $x$-comonoid $\phi = (x \stackrel{f}{\leftarrow} w \stackrel{f}{\rightarrow} x)$.
By assuming local cartesian closure,
we can prove \cite{Freyd} that $\widehat{\bf C}$ is standard cartesian.

When $\widehat{\bf C} = \pair{\widehat{\bf C}}{\directsquare{(\,)}{}}$ is a direct flow category,
the direct flow along any term $\term{y}{\rho}{x}$ decomposes as
$\directsquare{\rho}{}
 = \directsquare{r_0^{\rm op} \tprod r_1}{}
 = \directsquare{r_0^{\rm op}}{} \cdot \directsquare{r_1}{}
 = {\rm sub}_{r_0} \cdot \exists_{r_1}$, 
and satisfies the ``Beck condition''
$\exists_f \cdot {\rm sub}_g
 = \directsquare{f}{} \cdot \directsquare{g^{\rm op}}{}
 = \directsquare{f \tprod g^{\rm op}}{}
 = \directsquare{\hat{g}^{\rm op} \tprod \hat{f}}{}
 = \directsquare{\hat{g}^{\rm op}}{} \cdot \directsquare{\hat{f}}{}
 = {\rm sub}_{\hat{g}} \cdot \exists_{\hat{f}}$
for the pullback span
$y \stackrel{\hat{g}}{\leftarrow} \hat{x} \stackrel{\hat{g}}{\rightarrow} z$
of any opspan
$y \stackrel{f}{\rightarrow} x \stackrel{g}{\leftarrow} z$,
and when $\widehat{\bf C} = \pair{\widehat{\bf C}}{\inversesquare{(\,)}{}}$ is a inverse flow category,
the inverse flow along any term $\term{y}{\rho}{x}$ decomposes as
$\inversesquare{\rho}{}
 = \inversesquare{r_0^{\rm op} \tprod r_1}{}
 = \inversesquare{r_1}{} \cdot \inversesquare{r_0^{\rm op}}{}
 = {\rm sub}_{r_1} \cdot \forall_{r_0}$,
and satisfies the ``Beck condition''
$\forall_g \cdot {\rm sub}_f
 = \inversesquare{g^{\rm op}}{} \cdot \inversesquare{f}{}
 = \inversesquare{f \tprod g^{\rm op}}{}
 = \inversesquare{\hat{g}^{\rm op} \tprod \hat{f}}{}
 = \inversesquare{\hat{f}}{} \cdot \inversesquare{\hat{g}^{\rm op}}{}
 = {\rm sub}_{\hat{f}} \cdot \forall_{\hat{g}}$.

Generalizing from this,
a {\em hyperdoctrine (of comonoids)\/} $\quadruple{{\bf C}}{\exists}{{\rm sub}}{\forall}$
consists of
(1) a semiexact category {\bf C}, and
(2) two connected dialectical bases
    ${\bf C} \stackrel{{\rm C}^{(\,)}}{\longrightarrow} {\bf adj}$ and
    ${\bf C}^{\rm op} \stackrel{{\rm C}_{(\,)}}{\longrightarrow} {\bf adj}$,
where ${\bf C}^f = {\bf Sub}(y) \stackrel{\exists_f \dashv {\rm sub}_f}{\longrightarrow} {\bf Sub}(x)$
and   ${\bf C}_f = {\bf Sub}(x) \stackrel{{\rm sub}_f \dashv \forall_f}{\longrightarrow} {\bf Sub}(y)$
for any {\bf C}-arrow $y \stackrel{f}{\rightarrow} x$,
which satisfy either of the equivalent ``Beck conditions'' above.

Suppose that {\bf P} is a spannable join bisemilattice.
When {\bf P} has type sums,
$\widehat{{\bf P}^\dashv}$ is a join bisemilattice and 
$\widehat{{\bf P}^\dashv} \stackrel{\uterm{{\rm P}}{}}{\longrightarrow} {\bf P}$
is a morphism of join bisemilattices.
When {\bf P} is a spannable dialectical flow category with type sums,
we can define flow along functional spans $\widehat{{\bf P}^\dashv}$
in terms of flow along arbitrary {\bf P}-terms:
$\directsquare{\rho}{}
 \define \directsquare{\uterm{y}{x}(\rho)}{}
       = \directsquare{r_0^{\rm op} \tprod r_1}{}
       = \directsquare{r_0^{\rm op}}{} \cdot \directsquare{r_1}{}
       = {\rm sub}_{r_0} \cdot \exists_{r_1}$
for any functional span
$\rho = (y \stackrel{r_0 \dashv r_0^{\rm op}}{\leftharpoondown} r \stackrel{r_1 \dashv r_1^{\rm op}}{\rightharpoondown} x)$.
We automatically satisfy a generalized ``Beck condition''.
\begin{Proposition}
   \begin{enumerate}
      \item If {\bf P} is a spannable dialectical flow category with type sums,
         then ${\bf P}^\dashv$ is a hyperdoctrine of comonoids.
      \item If {\bf C} is a hyperdoctrine of comonoids,
         then $\widehat{{\bf C}}$ is a spannable dialectical flow category with type sums.
   \end{enumerate}
\end{Proposition}

\begin{Theorem}
   The spanning construction $\widehat{(\,)}$
   is left adjoint to
   the internal adjointness construction $(\,)^\dashv$
   \begin{center}
      \begin{tabular}{rcl}
         \begin{tabular}{c}
            Hyperdoctrines \\ of \\ Comonoids
         \end{tabular}
         &
         $\stackrel{\widehat{(\,)} \dashv (\,)^\dashv}{\longrightarrow}$
         &
         \begin{tabular}{c}
            Spannable \\ Dialectical Flow Categories \\ with Type Sums
         \end{tabular}
      \end{tabular}
   \end{center}
   with unit components given by the exact Yoneda embeddings 
   ${\bf C} \stackrel{{\rm y}_{\rm C}}{\longrightarrow} {\widehat{\bf C}}^\dashv$
   and counit components given by the underlying term biposet morphisms
   $\widehat{{\bf P}^\dashv} \stackrel{\uterm{{\rm P}}{}}{\longrightarrow} {\bf P}$.
\end{Theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Enriched Relations.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We discuss here in some detail another well-known (parametric) example of an assertional/flow category,
``enriched relations''.

Let {\bf V} = $\quadruple{V}{\preceq}{\otimes_V}{e}$
be any symmetric complete Heyting monoid. Such a poset is also called a {\em closed poset\/}.
Symmetry means commutativity of the tensor product $s \otimes_V r = r \otimes_V s$.
Consider the join bisemilattice (cHc)
${\bf Rel}_V = \distrib{\bf V} = \mat{\power{\bf V}}$
of ``{\bf V}-relations'' (see the definition of distributers below).
Since $\power{\bf V}$ is also a closed poset and $\power{\bf V} \neq {\bf 1}$,
we could equivalently consider $\mat{\bf W}$ for
${\bf W}$ a closed poset ${\bf W} \neq {\bf 1}$.
The special case {\bf V} = {\bf 1} is our most fundamental ``relational'' example of an assertional/flow category.
This is the cHc of ordinary relations
${\bf Rel} = {\bf Rel}_1 = \distrib{\bf 1} = \mat{\power{\bf 1}} = \mat{\bf 2}$,
the latter being matrices of booleans.
This example provides the standard semantics for dynamic logic.
The special cases ${\bf V} = {\bf 2'} = \langle \{1,0\},\geq,\vee,0 \rangle$ the datatype of ``booleans'',
and ${\bf V} = {\bf N} = \langle \{\infty,\cdots,1,0\},\geq,+,0 \rangle$ the ``natural numbers'' datatype,
are important in the logic of Petri nets:
{\bf V} = ${\bf 2'}$ for condition/event nets and
{\bf V} = {\bf N} for place/transition nets.
\begin{description}
   \item[horizontal aspect] \mbox{ }
      \begin{enumerate}
         \item A {\bf V}-type (an object of ${\bf Rel}_V$) is a pair $\pair{X}{|\;|_X}$,
            where $X$ is a set (of nodes, places or conditions)
            and $X \stackrel{|\;|_X}{\longrightarrow} \{e\}$ is a (trivial) typing function.
            So a type is just a set $X$.
            A {\bf V}-term $\term{Y}{r}{X}$ (an arrow of ${\bf Rel}_V$)
            is a $(\product{Y}{X})$-indexed function
            $\product{Y}{X} \stackrel{r}{\rightarrow} \power{V}$.
            So terms are matrices of subsets of {\bf V}-elements.
            Since $\power{\bf V}$ reflects into {\bf V} via the reflective pair of sup/principal-ideal monotonic functions
            $\power{\bf V} \stackrel{{\sqcup} \dashv {\downarrow}}{\longrightarrow} {\bf V}$,
            we can simplify terms to matrices with entries being {\bf V}-elements.
            We denote such a matrix $\term{Y}{r}{X}$ by $r = [r_{yx}] = [r_{yx} \memberof V \mid y \memberof Y, x \memberof X]$.
            Tensor product is matrix product
            $[s_{zy}] \tprod [r_{yx}] = [\bigsqcup_y (s_{zy} \otimes_V r_{yx})]$.
            The identity term at $X$ is the unit diagonal matrix $X = [X_{x'x}]$
            where $X_{x,x} = e \mbox{ when } x'=x, = 0_V \mbox{ when } x' \neq x$.
         \item Given any set $X$, a {\bf V}-object of type $X$ is a term $\term{1}{\phi}{X}$;
            or equivalently, an $X$-vector (row-matrix) $X \stackrel{\phi}{\rightarrow} V$
            or $\phi = [\phi_x \mid x \memberof X]$.
            {\bf V}-objects are also called
            ``{\bf V}-subsets'' for general {\bf V},
            ``markings'' when {\bf V} = {\bf N}, or
            ``cases'' when {\bf V} = ${\bf 2'}$.
            Let $\obj{}{(X)}{} \define V^X$ be the collection of all ${\bf V}$-objects.
            For any term $\term{y}{r}{x}$,
            the direct flow of objects
            $\obj{}{(Y)}{} \stackrel{\obj{}{}{r}}{\longrightarrow} \obj{}{(X)}{}$
            is defined by matrix product
            $\obj{}{(\psi)}{r} = \psi \tprod r$,
            and the inverse flow of objects
            $\obj{}{(Y)}{} \stackrel{\obj{r}{}{}}{\longleftarrow} \obj{}{(X)}{}$
            is defined by matrix quotient
            $\obj{r}{(\psi)}{} = \psi \tensorimplytarget r$.
            Endoterms $\term{X}{p}{X}$ are square matrices of size $X$,
            $p = [p_{x'x} \memberof V \mid x',x \memberof X]$.
            A {\bf V}-subobject $\term{X}{\phi}{X}$ of type $X$ is a diagonal matrix,
            $\phi = [\phi_{x'x}]$ where $\phi_{x'x} = 0_V \mbox{ if } x' \neq x$.
            For arbitrary closed poset {\bf V},
            {\bf V}-objects and {\bf V}-subobjects are isomorphic $\obj{}{(X)}{} \cong \subobj{}{(X)}{}$.
            Comonoids ({\bf V}-subtypes) are idempotent {\bf V}-subobjects;
            that is, diagonal matrices with terms on the main diagonal being idempotent {\bf V}-elements.
            Each square matrix (idempotent term) $\term{X}{p}{X}$ has an interior $\term{X}{\interior{p}}{X}$,
            which is the largest diagonal matrix of idempotent {\bf V}-elements below $p$;
            $\interior{p}_{xx} = \interior{(p_{xx})}$.
            So ${\bf Rel}_V$ is standard numeric for arbitrary {\bf V}.
            The closed poset {\bf V} is cartesian when tensor product $\tprod$ is ordinary product (meet) $\sqcap$;
            that is,
            when {\bf V} is a complete Heyting algebra.
            When {\bf V} is cartesian all elements are idempotent,
            and {\bf V}-subtypes are identical to {\bf V}-subobjects (diagonal matrices)
            and isomorphic to {\bf V}-objects (row matrices)
            $\obj{}{(X)}{} \cong \comonoid{}{X}{}$.
            So ${\bf Rel}_V$ is standard cartesian when {\bf V} is cartesian (a complete Heyting algebra).
      \end{enumerate}
   \item[vertical aspect] \mbox{ }
      \begin{enumerate}
         \item Term entailment and boolean sum are defined entrywise:
            $s \preceq_{YX} r$ when $s_{yx} \preceq r_{yx}$ for all $y \memberof Y$ and $x \memberof X$; and
            $[s_{yx}] \bsum_{YX} [r_{yx}] \define [s_{yx} \bsum_V r_{yx}]$.
            The bottom term between $Y$ and $X$ is the $\product{Y}{X}$ zero matrix.
         \item The closed poset ${\bf 2} = \quadruple{\{0,1\}}{\leq}{\wedge}{1}$
            can be embedded in to the closed poset ${\bf W} = \power{\bf V}$,
            $0$ as $0_W = \emptyset$ and $1$ as $e_W = \{e_V\}$.
            So any {\bf 2}-term is a $\power{\bf V}$-term.
            A {\bf V}-{\em morphism\/} is a {\bf 2}-term in ${\bf Rel}_V$
            which has the property:
            for each $y \memberof Y$ there is a unique $x \memberof X$ such that $r_{yx} = e_W$.
            So $r = [r_{yx}]$ is the ``graph'' of a unique function $Y \stackrel{f}{\rightarrow} X$,
            where $r_{yf(y)} = e_W$ and $r_{yx} = 0$ for $x \neq f(y)$.
            {\bf V}-morphisms are functional terms ${\bf Rel}_V$.
      \end{enumerate}
\end{description}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Standard Heyting Categories.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Loosely speaking,
a Heyting category {\bf H} is standard
when object flow restricts to (and hence extends) both subobject and subtype flow in a coherent fashion.
More precisely,
a Heyting category {\bf H} is said to be {\em standard\/}
when:
\begin{enumerate}
   \item it is an affirmation bisemilattice;
   \item for each type $x$,
         there is a coreflective pair of lattice morphisms
         between the Heyting algebra of subtypes and the lattice of objects
         $\comonoid{}{(x)}{} \stackrel{{o_x \dashv \sigma_x}}{\longrightarrow} \obj{}{(x)}{}$,
         where the object embedding satisfies the ``standardization axiom''
         \begin{center}
            $o_x(u) \tprod v = o_x(u \tprod v)$
         \end{center}
         for all subtypes $u,v \memberof \comonoid{}{(x)}{}$,
         or equivalently,
         the subtype coreflection satisfies
         $\phi \tprod \sigma_x(\psi) = \phi \wedge \psi$
         for all objects $\phi,\psi \memberof \obj{}{(x)}{}$;
   \item for each term $\term{y}{r}{x}$,
         there is an adjoint pair of monotonic functions
         between the source and target Heyting algebra of subtypes
         $\comonoid{}{(y)}{} \stackrel{{\comonoid{}{}{r} \dashv \comonoid{r}{}{}}}{\longrightarrow} \comonoid{}{(x)}{}$,
         which forms a commuting square of adjunctions with object flow and subtype/object coreflections
         \begin{center}
            $\begin{array}{rccccccl}
                & \comonoid{}{(y)}{} && \stackrel{\comonoid{r}{}{} \dashv \comonoid{}{}{r}}{\longrightarrow} & \comonoid{}{(x)}{} &&& \left. \mbox{\rule{0in}{.2in}} \right\} \mbox{``subtype flow''} \\
                && \searrow &&& \searrow && \\
                o_y \dashv \sigma_y & \downarrow && \multicolumn{1}{l}{\subobj{}{(y)}{}} & \stackrel{\subobj{}{}{r} \dashv \subobj{r}{}{}}{\longrightarrow} && \subobj{}{(x)}{} & \left. \mbox{\rule{0in}{.2in}} \right\} \mbox{``subobject flow''} \\
                && \swarrow &&& \swarrow && \\
                & \obj{}{(y)}{} && \stackrel{\obj{}{}{r} \dashv \obj{r}{}{}}{\longrightarrow} & \obj{}{(x)}{} &&& \left. \mbox{\rule{0in}{.2in}} \right\} \mbox{   ``object flow''}
             \end{array}$
         \end{center}
         or equivalently,
         satisfies either of the two equivalent conditions:
         \begin{center}
            $\begin{array}{p{1in}r@{\;=\;}lp{2.5in}}
                \mbox{\rule{1in}{0in}} & \comonoid{}{}{r} \cdot o_x      & o_y \cdot \obj{}{}{r}      & ``object flow extends subtype flow''      \\
                \mbox{\rule{1in}{0in}} & \sigma_x \cdot \comonoid{r}{}{} & \obj{r}{}{} \cdot \sigma_y & ``object flow restricts to subtype flow''
             \end{array}$
         \end{center}
\end{enumerate}
\begin{Proposition}
   A standard Heyting category {\bf H} defines a dialectical flow category,
   with flow of subtypes being restricted object flow.
\end{Proposition}
A Heyting category {\bf H} is said to be {\em standard numeric\/} ({\em standard cartesian\/})
when:
(1) it is an affirmation bisemilattice; and
(2) for each type $x$,
    there is an isomorphism
    between the lattices of subobjects (subtypes) and objects
    ${\bf Sub}(x) \cong \obj{}{(x)}{}$ ($\comonoid{}{(x)}{} \cong \obj{}{(x)}{}$),
    with isomorphism maps
    ${\bf Sub}(x) \stackrel{o_x}{\rightarrow} \obj{}{(x)}{}$
    and
    $\obj{}{(x)}{} \stackrel{\sigma_x}{\rightarrow} {\bf Sub}(x)$
    ($\comonoid{}{(x)}{} \stackrel{o_x}{\rightarrow} \obj{}{(x)}{}$
     and
     $\obj{}{(x)}{} \stackrel{\sigma_x}{\rightarrow} \comonoid{}{(x)}{}$),
    where the object isomorphism map satisfies
    $o_x(u) \tprod v = o_x(u \tprod v)$
    for all subobjects $\phi,\psi \memberof {\bf Sub}(x)$
    (subtypes $u,v \memberof \comonoid{}{(x)}{}$),
    or equivalently,
    the subobject (subtype) isomorphism map satisfies
    $\phi \tprod \sigma_x(\psi) = \phi \wedge \psi$
    for all objects $\phi,\psi \memberof \obj{}{(x)}{}$.
A standard numeric (standard cartesian) Heyting category {\bf H} {\em is\/} a dialectical flow category,
with flow of subtypes identified as object flow.



==> remember.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\rememberto
   {
   \begin{itemize}
      \item add fact that dialectical categories need no special axiom
         asserting existence of a local implication,
         since the local implication is induced by the inverse flow
         \begin{center}
            $u \imply v \define \inversesquare{u}{(v)}$;
         \end{center}
      \item {\bf Freyd's Theorem}
         define inverse flow by assuming existence of local implication 
         $u \imply v$;
         do this first for a semiexact category;
         next, do it for a spannable bisemilattice;
         finally, do it for an arbitrary join bisemilattice;
      \item review and correct two passages concerning partial functions;
      \item translate Goldblatt's section on $\Omega$-sets into dialectical logic;
      \item review coreflection between spannable bisemilattices
         and semiexact categories;
      \item smooth out the adjointness between {\em subtypes} and {\em comonoids},
         especially w.r.t. {\em domains} and {\em totalness};
      \item translate {\bf Rel} definition of quantifiers
         to arbitrary join bisemilattices;
      \item ${\rm sub}_{r_0}$ preserves pullbacks,
         $\exists_{r_1}$ preserves composition,
         {\em so} $\cdots$;
      \item Heikka's translation procedure;
      \item embed Meseguer-Montanari approach to nets into dialectical logic;
   \end{itemize} 
   }


